Universal Approximation Under Constraints is Possible with Transformers

Many practical problems need the output of a machine learning model to satisfy a set of constraints, $K$. Nevertheless, there is no known guarantee that classical neural network architectures can exactly encode constraints while simultaneously achieving universality. We provide a quantitative constrained universal approximation theorem which guarantees that for any non-convex compact set $K$ and any continuous function $f:\mathbb{R}^n\rightarrow K$, there is a probabilistic transformer $\hat{F}$ whose randomized outputs all lie in $K$ and whose expected output uniformly approximates $f$. Our second main result is a "deep neural version" of Berge's Maximum Theorem (1963). The result guarantees that given an objective function $L$, a constraint set $K$, and a family of soft constraint sets, there is a probabilistic transformer $\hat{F}$ that approximately minimizes $L$ and whose outputs belong to $K$; moreover, $\hat{F}$ approximately satisfies the soft constraints. Our results imply the first universal approximation theorem for classical transformers with exact convex constraint satisfaction. They also yield that a chart-free universal approximation theorem for Riemannian manifold-valued functions subject to suitable geodesically convex constraints.

==> Rebuttals.tex <==
%%%% This document contains the rebuttals to each of the ICLR Referees  %%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             Rebuttals:                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%=====================%
%---------------------%
%%%%% Reviewer 1 %%%%%%
%%%% Reviewer VnD6 %%%%
%---------------------%
% who awarded us an 8 %
%=====================%

Thank you for your positive review and suggestions to further improve the manuscript. As a general comment, in the updated manuscript we made an earnest effort to hunt down typos and add discussions that improve clarity (also in response to other reviewers' comments). 

*Is there any connection that can be said in this case under Ricci curvature tensor?*

**Response:** 
This is an intriguing thought.  The main property which Assumption 2.10 gave us is strict convexity of the integral functional in Equation 9 (as a function of $\mathbb{P}$) and Lipschitz-continuity of its argmin.  In other words, the "Wasserstein barycenter-map" sending $\mathbb{P}\in \mathcal{P}_1(K)$ to $\overline{\mathbb{P}}\in K$ should be well-defined and Lipschitz.  Though there is little work in the optimal transport of metric geometry literature on the topic, we are aware of the paper by Kim et al. "Wasserstein barycenters over Riemannian manifolds" (2017), specifically Corollary 7.12, which could possibly be used to establish an analogue to Lemma C.3.  Thus, we believe that a generalization of Corollary 2.11 replacing sectional curvature bounds by the less restrictive Ricci curvature bounds is possible. However, it would require some time due to the involved technical subtleties.  

In terms of generalizations and extensions of the framework considered here in this paper, our next/current goal (in a follow-up work which we have already begun) is to derive an infinite-dimensional version of our results that can handle functional constraints.  Applications of such a follow-up result may be found, for example, to fairness in machine learning, quantitative risk management (constraints via convex functionals; see McNeil et al. (2015) "Quantitative Risk Management"), or robust learning (Javed et al. (2021) "Policy Gradient Bayesian Robust Optimization for Imitation Learning"), all in connection to the coherent risk-measures introduced by Artzner et al. "Coherent Measures of Risk" (1999).  


*It would be a good idea to provide more examples to demonstrate the general theory.*

**Response:** 
We agree that additional examples and illustrations could further improve the paper. We have therefore included a discussion on page $1$ citing examples of manifold constraints arising in robotics, computer vision, and in mathematical finance. We also expanded our numerical experiments to illustrate the variety of geometries addressed by our theory (from convex sets to manifolds to certain ``pathological'' constraint sets). Finally, we promoted the section with numerics from Appendix E to Appendix B.  All these changes are written in teal blue.  

We hope that the new discussions, experiments, and illustrations address your comments.


%=====================%
%---------------------%
%%%%% Reviewer 2 %%%%%%
%%%% Reviewer w3Aa %%%%
%---------------------%
% who thinks we're 3  %
%=====================%
We thank the reviewer for their valuable feedback.  We, however, respectfully disagree with most of the critical points raised. We hope to articulate why below. 

*“The paper is hard to follow at many places since only informal theorems are provided throughout the paper”.  *(later)* “[A]ll the technical statements in the main paper are Informal theorems with no rigorous explanations provided”.*

**Response:**
This is not the case: A rigorous version of all statements are given in Section 2 (Theorem 2.2, Corollary 2.3, Theorem 2.7, Corollary 2.8, Corollary 2.9 and Corollary 2.11) on pages 7-9. The rationale behind first stating informal versions is actually to make the exposition clearer and to begin by explaining the intuition and operational meaning (as pointed out by Reviewer VnD6). A similar strategy is adopted by many other theory-forward machine learning papers. (We note that a version of Table 1 with explicit constants is provided in Appendix A (Table 2).)

*“Somewhat related to the previous point, some technically deep concepts (such as Wasserstein-1 distance) are introduced in passing and handled in a slightly cavalier manner”.*

**Response:**
The Wasserstein-$1$ distance was indeed used in Section 1.2 before being formally defined in Section 1.4. Thank you for catching this. We have added a reference to section 1.4.

*“It could have been nice if the authors provided some explanations to the figures -- at the moment, the reader has to guess what the authors intend to say.”*

**Response**
We have added further explanations following Figures 1-2 and Figures 3-4. You can find the modifications in teal blue.

*“The main theorem 2.2 is suboptimal -- optimal network may require width greater than the number of input dimensions n. For image analysis, this corresponds to the number of pixels.”*

**Response:**
For small $\epsilon$ the complexity estimates in Table 1 imply that the encoder and decoder networks' widths are indeed *larger* than the input dimension. We realized that the confusion might have arisen from ``flipped'' ordering of the columns in Table 1; in the revised version we swapped the columns to make this clearer. The encoder network's width is lower-bounded by the input dimension $n$ and the decoder's width depends on $\frac{1}{\epsilon}$.

*The constraint examples are too unnatural.*

**Response:**
In Sections 2.3.1 and 2.3.2 (Corollary 2.9 and Corollary 2.11) we derive constrained universal approximation guarantees for any convex constraint and a broad range of non-convex but geodesically-convex cases.  This covers many examples in convex and non-convex optimization including linear, quadratic, or semi-definite constraints. It also covers instances of geometric deep learning between Riemannian manifolds of interest in computer vision, structured matrix-valued learning, and information theory/information geometry, to name a few. It includes as special cases classes of matrices such as unitary matrices, covariance matrices, or distance matrices; pose manifolds in robotics, functions on spheres, tori spaces, and many other sets and spaces used in modern machine learning. All of these examples arise naturally in a variety of applications from computer vision and robotics to operations research to mathematical finance. We emphasize that our theory also admits arbitrary constraint sets much beyond these familiar examples. 
Your comment made us realize that these facts and connections should be further emphasized; we included a  discussion on page $1$ in the updated manuscript.

*[I]n geometric deep learning, authors argue that when K is a disjoint set, then the closest point computation becomes an unmanageable dilemma, claiming that the linear relaxations are meaningless for integer program (IP) while LPs are routinely used to solve IPs in practice using a branch and bound scheme.*

**Response**
We use disconnected sets as an example of extremes covered by out theory; our main geometric deep learning results concern the problem of approximating functions that take values in a Riemannian manifold (Section 2.3.2, esp. Corollary 2.11). These results show that when the constraint set $K$ is a geodesically convex subset of a (complete) Riemannian manifold, universal approximation of a $K$-valued function is possible with a transformer which takes values in $K$. We emphasize that, unlike the motivational discussion about integers, our results about manifolds are of central interest in geometric deep learning (e.g., the survey papers: M. Bronstein et al. (2017) "Geometric deep learning: going beyond Euclidean data" Section 4 and Section 4.4 of M. Bronstein et al. (2021) " Geometric Deep Learning: Grids, Groups, Graphs, Geodesics, and Gauges"). Furthermore, our results are the only available chart-free guarantees (Corollary 2.11) in this direction.

You are right that LPs (perhaps combined with branch-and-bound) may be used to approximate (or exactly solve) certain (mixed-)integer programs. But our paper is (among many other things) about universally approximating solution maps to such constrained problems by neural networks. (*) The integer example serves only to illustrate a technical obstruction whose removal requires a new mathematical idea. We give first existing results in this direction. We emphasize that integer constraints are only a very specific instance of the broad class of constraints handled by our results (from familiar constraints like polytopes to bizarre constraints like disjoint unions of sets of different dimension), most of which do not admit any known mathematical programming technique. 

*[T]here are many confusing notations at various places that can easily be avoided - "Attention" in eq (4) is different from "attention".*

**Response:**
With this notation we tried to emphasize the strong link between the two concepts (Equation (4)), but we now realize that it may be quite confusing. We thus replaced ``attention'' by $P-\operatorname{attention}$. We also scanned the manuscript for other possibly confusing notation. If there is anything in particular you find problematic please let us know.

*Given that the paper shows quantitative results in the infinite sample setting, it is not clear whether the results hold in the finite sample setting where transformers are being used in practice.*

**Response:**
Our paper indeed derives a universal approximation guarantee and not a statistical guarantee (such as a bound on the generalization gap). In this sense, our main statement adds to the line of work spearheaded by Hornik et al. in "Multilayer feedforward networks are universal approximators" (1989) and Cybenko "Approximation by superpositions of a sigmoidal function" (1989) and parallels recent sophisticated versions for networks on graphs (Kerien et al. "Universal Invariant and Equivariant Graph Neural Networks" (2019)), networks that obey symmetries specified by certain groups (Yarotsky "Universal approximations of invariant maps by neural networks" (2021)), etc. Statistical guarantees are important but complementary to our results and they require a rather different set of techniques, see for instance: Alquier et al. "On the properties of variational approximations of {G}ibbsposteriors" (2016) or Ribeiro et al. "Probably approximately correct constrained learning" (2020).


*No experiments to verify any of the quantitative results.*

**Response:**
We agree with that stylized numerical experiments may help validate our quantitative theoretical claims. In the new Section B.3 we set out to probe the main new quantitative statement in Theorem 2.2. Namely, we confirm that ``The model complexities in Table 1 are independent of $K$'s geometry''. We do so by approximating various functions taking values in a constraint set whose geometry is made progressively more complicated, beginning with a polytope, moving to a nonpolytopal convex set, then to a manifold, and eventually to a ``degenerate'' non-convex set which is not a manifold.  The depth and width of the approximating architecture are fixed across all experiments in order. We find that the probabilistic transformer implementing the approximation indeed performs comparably across all geometries relative to the MLP.

Let us add that, a priori, our results guarantee existence of a choice of weights such that the proposed network approximates any admissible target function with a desired accuracy, but they do not tell us how to find those weights. How to do this with guarantees is largely an open question at the interface of statistics and (non-convex) optimization theory. Such empirical verifications thus have to be interpreted with care. That is the reason why recent papers on universal approximation (e.g., Kidger et al. (2020) "Universal Approximation with Deep Narrow Networks," S. Park et al. (2021) "Minimum Width for Universal Approximation," etc..) refrain from reporting numerical results.

*It would have been nice if the authors can formulate and show some toy experiments to even check whether such universality may be possible for dataset in the hands of a practitioner.*

**Response:**
Similarly to prior universal approximation results (classics + recent ICLR papers) ours puts forward a theoretical guarantee. Although numerical experiments are uncommon in these papers, we agree that some amount of experimental evidence is valuable (in line with our response to your previous comment). We thus included preliminary numerics in .... . To further strengthen this aspect, in the revised manuscript .... . We feel that adding many more numerical results would shift the focus away from the core contribution.


%=====================%
%---------------------%
%%%%% Reviewer 3 %%%%%%
%%%% Reviewer tJ9y %%%%
%---------------------%
%=====================%

Thank you taking the time to review our paper. We are very pleased that you enjoyed it!

*On the attention module. I: I think the paper could benefit from further explaining why this particular form of attention is natural. It would also perhaps help to illustrate this with an example. As the credibility of the paper relies on the reader accepting that this attention model is natural and general enough to form the basis of the approach to universal approximation, I think that it's worth spending some more time here. In particular, I didn't get a good sense of the role of the matrix in build up to Informal Theorem 1.*

**Response:** 
This is a very good point and we hope that it is addressed by our modified version of the manuscript and its appendices. We added to the discussion following Figure $1$ as well as a discussion in the new Appendix B.3 section (which is integrated into page 14 following Figures $6$ and $7$) explaining why this form of attention is natural for our problem.  We have also included additional numerical illustrations in the same appendix section which we hope help convince the reader both of the suitability of this form of attention to the problem of approximation under constraints, for constraints ranging between convex to highly non-convex. In Figure $1$, when $K$ is a convex polytope then these ``particles'' $Y_1,\dots,Y_N$ are placed on $K$'s vertices and in general (Appendix B.3.2) these particles are placed all over $K$.  



*Figures. Don't get me wrong, I love that there are figures here. However, I think that they could be explained better. For instance, it wasn't clear to me what the green region was in Figure 1. Is this?*
*Also, the blue dot seems too small, and thus quite hard to see. *

**Response:** 
Based on your suggestions, as well as those of reviewers #1 (VnD6) and #2 (w3Aa), we have expanded the figure descriptions in the text.  The green part of Figure 1 represents $K$, the purple dots represent the ``particles'' $Y_1,\dots,Y_N$, the size of the violet bubble around each particle illustrates the probability that it is predicted by the probabilistic transformer, and the blue dot is the weighted average of these particles.  Thus, the blue dot (which we enlarged) corresponds to the output of the deterministic transformer.  Moreover, we took the opportunity to re-draw the illustrations in Figures 3 and 4, they should be clearer than before.  Thanks for pointing this out.  

Thank you again for your encouraging assessment and helpful feedback.  









%=====================%
%---------------------%
%%%%% Area Chair %%%%%%
%---------------------%
%=====================%
        %% A:  Ivan's magic is definitely needed here ;)
Dear Area Chair,

We know that you are very busy at this time.  
We are only briefly reaching out to bring to your attention that reviewer (w2Aa on Paper 3390) has likely not read our manuscript past the introduction, as is evidenced by their many false claims.  We, of course, understand that there can be a random component to any machine learning conference but, seeing as their review is fully at odds with the others (8 and 10) we only hope that by bringing this issue to your attention to calibrate our paper's SnR.


Dear Area Chair,

We know that you are very busy at this time.  
We are only briefly reaching out to bring to your attention to the review provided by reviewer w2Aa on Paper 3390.  The reviewer has many objections to our paper to which we answered thoroughly. We also made our best effort to improve the paper and resolve the many misunderstandings in the shortest amount of time possible. However, they have neither replied nor have updated their review after passing of two weeks despite the official recommendation for a 3-day feedback. 

 We, of course, understand that that the revoewers can busy at this time but seeing as their review is fully at odds with the others (8 and 10) we only hope that by bringing this issue to your attention to calibrate our paper's SnR.










%%%%%%%%% 
% S. Biderman
% COMMENT 1
We are approximating $f:\mathbb{R}^n\rightarrow K$ by passing the Wasserstein space. By viewing it as a function in $\mathbb{R}^n \rightarrow \mathcal{P}_1(K)$, this lifting to probability measures allows us to delete all topological obstructions (see Theorem 6 in A. Kratsios and L. Papon's paper ``Universal Approximation Theorems for Differentiable Geometric Deep Learning''). Thus the width of any such model must grow since $\mathcal{P}_1(K)$ is infinite-dimensional (by way of analogy, the universal approximation theorems for *feedforward networks* between Euclidean spaces (such as Park et al. 2021 ICLR paper `Minimum Width for Universal Approximation’’ or P. Kidger and T. Lyons 2020 NeurIPS paper "Universal Approximation with Deep Narrow Networks") require the width to grow proportionally to the input and output dimensions; this is the same in our case).

That said, the rates we derive in Table 1 (and Table 2 in the appendix) show that our approximating transformer’s depth and width both scale as a function of the approximation accuracy.  In particular, its depth scales faster than its width.  This seems to confirm and reflect the experimental evidence, which you refer to, that a transformer’s depth is more expressive than its width.

To address the final question, we do in fact believe that when K is a convex polytope then the approximating transformer can be taken to have fixed width, proportional to the number of K’s vertices, and only its depth scales as a function of the approximation quality.  We did not include this case since the same reasoning does not apply to general convex sets, and, perhaps more interestingly, to general non-convex K.

% COMMENT 2
The interpretation of $Y$ in our setting is as an array of ``particles’' on the constraint set $K$.  There are certainly many problems successfully addressed by bespoke versions of attention. For the question of constrained universal approximation, the formulation we use (and its probabilistic variant in Equation (3)) is appealing since it has a simple interpretation, is easy to write down in practice, and allows us to leverage probabilistic tools.
